Modular abstract syntax trees (MAST): substitution tensors with second-class sorts

We adapt Fiore, Plotkin, and Turi's treatment of abstract syntax with binding, substitution, and holes to account for languages with second-class sorts. These situations include programming calculi such as the Call-by-Value lambda-calculus (CBV) and Levy's Call-by-Push-Value (CBPV). Prohibiting second-class sorts from appearing in variable contexts changes the characterisation of the abstract syntax from monoids in monoidal categories to actions in actegories. We reproduce much of the development through bicategorical arguments. We apply the resulting theory by proving substitution lemmata for varieties of CBV.

==> misc-tensorial-proofs.tex <==
\section{}


==> preamble.tex <==
\usepackage{enticsmacro}
\usepackage{graphicx}
\usepackage[all]{xy}
\usepackage{url}
\sloppy
% The following is enclosed to allow easy detection of differences in
% ascii coding.
% Upper-case    A B C D E F G H I J K L M N O P Q R S T U V W X Y Z
% Lower-case    a b c d e f g h i j k l m n o p q r s t u v w x y z
% Digits        0 1 2 3 4 5 6 7 8 9
% Exclamation   !           Double quote "          Hash (number) #
% Dollar        $           Percent      %          Ampersand     &
% Acute accent  '           Left paren   (          Right paren   )
% Asterisk      *           Plus         +          Comma         ,
% Minus         -           Point        .          Solidus       /
% Colon         :           Semicolon    ;          Less than     <
% Equals        =3D           Greater than >          Question mark ?
% At            @           Left bracket [          Backslash     \
% Right bracket ]           Circumflex   ^          Underscore    _
% Grave accent  `           Left brace   {          Vertical bar  |
% Right brace   }           Tilde        ~

%%%%%%%%	Your Corresponding Editor will provide the following information:
\def\conf{MFPS 2025}
\volume{NN}			%Fill in the ENTICS volume number here
\def\volu{NN}			% and here
\def\papno{nn}			%Fill in your paper number here
%%%%%%%%Please fill in the following information:
\def\lastname{Kammar, Moser, and Staton} %Lastnames appear in the running header
\def\runtitle{Modular abstract syntax trees} %Short title appears in the running header on even pages.
%%
\def\copynames{O. Kammar and G. Moser}

\def\CCB{CC@symbol}

\newcommand\authoremail[2]{
  \thanks[#1]{Email: \href{mailto:#2} {\texttt{\normalshape
        #2}}}}

\input{defs}

